Adversarial Examples in Constrained Domains

Machine learning algorithms have been shown to be vulnerable to adversarial manipulation through systematic modification of inputs (e.g., adversarial examples) in domains such as image recognition. Under the default threat model, the adversary exploits the unconstrained nature of images; each feature (pixel) is fully under control of the adversary. However, it is not clear how these attacks translate to constrained domains that limit which and how features can be modified by the adversary (e.g., network intrusion detection). In this paper, we explore whether constrained domains are less vulnerable than unconstrained domains to adversarial example generation algorithms. We create an algorithm for generating adversarial sketches: targeted universal perturbation vectors which encode feature saliency within the envelope of domain constraints. To assess how these algorithms perform, we evaluate them in constrained (e.g., network intrusion detection) and unconstrained (e.g., image recognition) domains. The results demonstrate that our approaches generate misclassification rates in constrained domains that were comparable to those of unconstrained domains (greater than 95%). Our investigation shows that the narrow attack surface exposed by constrained domains is still sufficiently large to craft successful adversarial examples; and thus, constraints do not appear to make a domain robust. Indeed, with as little as five randomly selected features, one can still generate adversarial examples.

==> adaptive_jsma.tex <==
\section{Adaptive JSMA}
\newcommand\bff{\boldsymbol{F}}
\newcommand\bigone{\,\,1\,\,}
\newcommand\onevector{\begin{pmatrix}
  \bigone \\ \bigone \\ \vdots \\ \bigone  
\end{pmatrix}}
\makeatletter
\newcommand*\dashline{\rotatebox[origin=c]{90}{$\dabar@\dabar@\dabar@$}}
\makeatother
%
\subsection{Formulation of Adaptive JSMA with Papernot's notation}
\begin{algorithm}
  \DontPrintSemicolon
  \SetKwInOut{Input}{Input}
  \Input{$\nabla F(X)$, $\Gamma$, $t$}
  % $\mu = -\nabla F(X)_t \odot ( \nabla F(X)_{\neg t} \mathbf{1} )$\\
  $\mu = - [ \nabla F_{\neg t}(X) \, \mathbf{1} ] \odot \nabla F_t (X) $\\
  $\textrm{mask} = (\mu > \mathbf{0})$\\
  $S = \mu\odot \textrm{mask} \odot \Gamma$\\
  $i_{\textrm{max}}=\textrm{arg max}_i \, S_i$\\
  % \textbf{return} $i_{\textrm{max}}, \sign{(\nabla F_{i,t})}$\\
  \textbf{return} $i_{\textrm{max}}, \sign{(\nabla F_{i,t}(X))}$\\
  \caption{\textsc{Adaptive JSMA Subroutine} \newline
  \label{alg:ajsma:alt}
  \textbf{$\nabla F$} is the Jacobian for a given sample $X$,
  \textbf{$\Gamma$} is a mask of the search domain, \textbf{$t$} is
  the target class.}  \algorithmfootnote{In this paper, we adapt the
    convention of \cite{papernot2016limitations} to express the
    Jacobian matrix $\nabla F(X) = \frac{\partial F}{\partial X}$ as
    an $m$ by $n$ matrix, the $(i,j)^\textrm{th}$ entry is $\frac{\partial
      F_j}{\partial X_i}$.  We express all of our vectors as column
    vectors.  The vector of inputs, $X$, is a 1 by $m$ vector, where
    $n$ is the number of features, e.g., pixels in images. We denote
    $\neg t$ to be all classes other than class $t$ and $\odot$ to be
    element-wise multiplication.  Finally, we define $\mathbf{1}$ to
    be a vector of 1's of length $\lvert \neg t \rvert$.}
\end{algorithm}
%
\subsection{Our original formulation of Adaptive JSMA}
\begin{algorithm}
  \DontPrintSemicolon
  \SetKwInOut{Input}{Input}
  \Input{$\nabla \bff(X)$, $\Gamma$, $t$}
  $\mu = -\nabla \bff(X)_t \odot (\mathbf{1}^T \nabla \bff(X)_{\neg t}) $\\
  $\textrm{mask} = (\mu > \mathbf{0})$\\
  $S = \mu\odot \textrm{mask} \odot \Gamma$\\
  $i_{\textrm{max}}=\textrm{arg max}_i \, S_i$\\
  \textbf{return} $i_{\textrm{max}}, \sign{(\nabla \bff(X)_{t,i})}$\\
  \caption{\textsc{Adaptive JSMA Subroutine} \newline
  \label{alg:ajsma}
  \textbf{$\nabla \bff$} is the Jacobian for a given sample $X$,
  \textbf{$\Gamma$} is a mask of the search domain, \textbf{$t$} is
  the target class.}  \algorithmfootnote{For the purposes of
    mathematical notation in this paper, and without loss of
    generality, we assume that $X$ is a 1 by
    \color{red} $m$ \color{black} vector, where $n$ is the number of
    features e.g., pixels in images. We denote $\neg t$ to be all
    classes other than class $t$ and $\odot$ to be element-wise
    multiplication.  Finally, we define $\mathbf{1}$ to be a column
    vector of 1's of length $\lvert \neg t \rvert$.}
\end{algorithm}
%
\section{Papernot notation} % \usepackage{amssymb}
%
\noindent $F: \mathbb{R}^m \rightarrow \mathbb{R}^n$ \\
$J_F(X) = \nabla F(X) =\left( \frac{\partial F_j}
{\partial X_i}\right)_{i=1\cdots m, j =  1\cdots n}$\\
$ X_{m \cdot 1} = \begin{pmatrix} X_1\\ \vdots \\ X_m \end{pmatrix}$, \quad
$\mathbf{1}_{(n-1)\cdot 1} =
\onevector$\\
$\nabla F(X)_{m \cdot n}$\\
$\nabla F_t(X)_{m \cdot 1}$\\
$\nabla F_{\neg t}(X)_{m \cdot (n-1)}$\\
\begin{equation*}
  \begin{aligned}
  \nabla F(X) & =
  \begin{pmatrix}
    %
    \frac{\partial F_1}{\partial X_1} & 
    \frac{\partial F_2}{\partial X_1} &
    \cdots &
    \frac{\partial F_n}{\partial X_1} \\
    %
    \frac{\partial F_1}{\partial X_2} & 
    \frac{\partial F_2}{\partial X_2} &
    \cdots &
    \frac{\partial F_n}{\partial X_2} \\
    %
    \vdots & \vdots & \ddots & \vdots \\
    %
    \frac{\partial F_1}{\partial X_m} & 
    \frac{\partial F_2}{\partial X_m} &
    \cdots &
    \frac{\partial F_n}{\partial X_m} \\
    %
  \end{pmatrix}\\
  & = \begin{pmatrix}
    \nabla F_1(X) & \dashline & \nabla F_2(X) & \dashline & \cdots & \dashline & \nabla F_n(X)
  \end{pmatrix}
  \end{aligned}
\end{equation*}
%
% \newpage
\section{Comparison of JSMA and AJSMA}
For AJSMA, we want (compare equation (9) in \cite{papernot2016limitations}):\\
\begin{equation*}
  \begin{aligned}
    S & = J_{i,t}(X)|\sum_{j\ne t}J_{i,j}(X)|
    =\nabla F_{i,t}(X)|\sum_{j\ne
    t}\nabla F_{i,j}(X)| \\
%  & \textrm{ whenever }\nabla F_{i,t}(X) <0 \textrm{ and }
%  \sum_{j\ne t}\nabla F_{i,j}(X) >0,
  & \textrm{ whenever }\nabla F_{i,t}(X) \sum_{j\ne t}\nabla F_{i,j}(X)  < 0,
  \\
  & \textrm{ and } S= 0 \textrm{ otherwise.}
  \end{aligned}
\end{equation*}
\noindent For this example, without (much) loss of generality, let's take $t$ to
be the $n^\textrm{th}$ class so that $\neg t = \{ 1,2,\hdots, n-1 \}$.

\begin{equation*}
  \begin{aligned}
    \nabla F_{\neg t}(X) \, \mathbf{1} & = 
    \begin{pmatrix}
      \nabla F_1 & \dashline & \nabla F_2 & \dashline & \cdots & \dashline & \nabla F_{n-1}
    \end{pmatrix}
    \onevector\\
    & = 
    \begin{pmatrix}
      \sum_{j \ne t} \nabla F_{1,j} \\
      \sum_{j \ne t} \nabla F_{2,j} \\
      \vdots\\
      \sum_{j \ne t} \nabla F_{m,j} \\
    \end{pmatrix}
  \end{aligned}
\end{equation*}

\noindent The $i^\textrm{th}$ element is $\sum_{j \ne t} \nabla F_{i,j}$.

\begin{equation*}
  \mu_i = - \left\{ [ \nabla F_{\neg t}(X) \, \mathbf{1} ] \odot \nabla F_t (X) \right\}_i
     = - \nabla F_{i,t} \sum_{j \ne t} \nabla F_{i,j}
\end{equation*}
%
\noindent JSMA requires
\begin{equation*}
  \textrm{mask } = (\mu>0) \wedge (\nabla F_t (X) <0),
\end{equation*}
AJSMA requires
\begin{equation*}
  \textrm{mask } = (\mu>0).
\end{equation*}


\bibliographystyle{IEEEtranS}
% \bibliography{bibliography-sheatsley} 
\bibliography{references}


==> algorithms.tex <==
\newpage
\section{Algorithms} \label{sec:algorithms}

\begin{algorithm}
  \DontPrintSemicolon
  \SetKwInOut{Input}{Input}
  \Input{$\nabla F(X)$, $\Gamma$, $t$}
  % $\mu = -\nabla F(X)_t \odot ( \nabla F(X)_{\neg t} \mathbf{1} )$\\
  $\mu = - [ \nabla F_{\neg t}(X) \, \mathbf{1} ] \odot \nabla F_t (X) $\\
  $S = \mu\odot \varphi_{\mu>0}(\Gamma)$\\
  % $\textrm{mask} = (\mu > \mathbf{0})$\\
  % $S = \mu\odot \textrm{mask} \odot \Gamma$\\
  $i_{\textrm{max}}=\textrm{arg max}_i \, S_i$\\
  % \textbf{return} $i_{\textrm{max}}, \sign{(\nabla F_{i,t})}$\\
  \textbf{return} $i_{\textrm{max}}, \sign{(\nabla F_{i,t}(X))}$\\
  \caption{\textsc{Adaptive JSMA Subroutine} \newline
  \label{alg:ajsma:alt}
  \textbf{$\nabla F$} is the Jacobian for a given sample $X$,
  \textbf{$\Gamma$} is the search domain, \textbf{$t$} is
  the target class.}  \algorithmfootnote{In this paper, we adapt
    Papernot's \cite{pp16limit} convention to express
    the Jacobian matrix $\nabla F(X) = \frac{\partial F}{\partial X}$
    as an $m$ by $n$ matrix, the $(i,j)^\textrm{th}$ entry is
    $\frac{\partial F_j}{\partial X_i}$.  We express all of our
    vectors as column vectors.  The vector of inputs, $X$, is a 1 by
    $m$ vector, where $n$ is the number of features, e.g., pixels in
    images. We denote $\neg t$ to be all classes other than class $t$
    and $\odot$ to be element-wise multiplication.  We define
    $\mathbf{1}$ to be a vector of 1's of length $\lvert \neg t
    \rvert$.  Finally, the mask $\varphi_A(X)$ is defined to be the
  predicate $A \subset X$ \cite{minskypapert}.}
\end{algorithm}

\begin{algorithm}
  \DontPrintSemicolon
  \SetKwInOut{Input}{Input}
  \Input{H, n}
  $v = \mathbf{\emptyset}$\\
  \While{$\textrm{\upshape dim } v \neq n$} 
  {
    $i=\textrm{arg max } \lvert H_i \rvert$\\
    $v=\textrm{append}(v, (i, \textrm{sign}(H_i)))$\\
    $H_i=0$\\
  }
  \textbf{return} $v$
  \caption{\textsc{Top-n Approximation\newline}
  \label{alg:top_n}
  $H$ is a perturbation histogram, $n$ is the desired number of features
  used to build the universal perturbation vector, $v$.
  }
  \algorithmfootnote{The vector $v$ is initialized to the $0$-dimensional ``empty vector'' 
which we denote by $\mathbf{\emptyset}$.  At each step of the \textbf{while} loop, the index 
and direction of the feature resulting in the $k^{\textrm{th}}$ largest perturbation is appended to $v$.}
\end{algorithm}

